Fully Abstract Normal Form Bisimulation for Call-by-Value PCF

We present the first fully abstract normal form bisimulation for call-by-value PCF (PCF$_{\textsf{v}}$). Our model is based on a labelled transition system (LTS) that combines elements from applicative bisimulation, environmental bisimulation and game semantics. In order to obtain completeness while avoiding the use of semantic quotiening, the LTS constructs traces corresponding to interactions with possible functional contexts. The model gives rise to a sound and complete technique for checking of PCF$_{\textsf{v}}$ program equivalence, which we implement in a bounded bisimulation checking tool. We test our tool on known equivalences from the literature and new examples.

==> SC.tex <==
\section{Proof of \cref{theorem:SC}}\label{sec:sound-complete}

We let a \emph{trace} be a sequence of app and ret moves (i.e.\ labels), as defined in  \cref{fig:lts}. A trace is \emph{complete} if it is starts with a fully bracketed segment, followed by a proponent return and is afterwards again fully bracketed, i.e.\ it adheres to the grammar:
\begin{align*}
  CT &::= \ Y\,\lpropret{D}\,X\\
  X  &::= \ \varepsilon\mor\lopapp{\alpha}{D}\ Y\,\lpropret{D}\,X\\
  Y  &::= \ \varepsilon\mor\lpropapp{\alpha}{D}\ X\,\lopret{D}\,Y
\end{align*}


\begin{theorem}[\cite{Laird07}]\label{theorem:FA}
Expressions $\vdash e_1: T$ and $\vdash e_2: T$ are contextually equivalent iff the configurations
  $\conf{\emptyA}{\emptyG}{\emptyK}{\emptyS}{e_1},
  \conf{\emptyA}{\emptyG}{\emptyK}{\emptyS}{e_2}$ produce the same complete traces.
\end{theorem}

\paragraph{Proof of \cref{theorem:SC}}
We first note that our LTS is deterministic modulo the selection of fresh locations in tau transitions. Moreover,
by \cref{theorem:FA}, it suffices to show that $e_1,e_2$ are bisimilar iff they have the same complete traces.

If the two expressions have the same complete traces then each of them can match any challenge posed by the other, so long as such a challenge can lead to a complete trace. If a challenge is doomed to not complete, then it can be matched by a transition to $\botconf$. 
Conversely, if $e_1,e_2$ are bisimilar then any transition sequence yielding a complete trace of $e_1$ can be simulated by $e_2$, and vice versa, so the two expressions have the same complete traces.\qed
 
\begin{remark}
  Soundness is also proved via the up to techniques in \cref{sec:soundness}.
  Completeness is also proved directly in \cref{sec:completeness}.
\end{remark}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> apx-games.tex <==
% An attempt to prove full abstraction via the innocent game model
% There is a lot of infrastructure to be introduced and then the correspondence
% with the trace model would need to be proven, which would be very tedious.

\newcommand\view[1]{\mathsf{view}(#1)} 	
\newcommand\pview[1]{\ulcorner#1\urcorner} 	
\newcommand\oview[1]{\llcorner#1\lrcorner} 	
\newcommand\ang[1]{\langle#1\rangle}
\newcommand\ini{\mathtt{i}}
\newcommand\que{\mathtt{q}}
\newcommand\ans{\mathtt{a}}
\newcommand\To{\Rightarrow}
\newcommand\rest{\upharpoonright}
\newcommand\sem[1]{\llbracket  #1\rrbracket}
\newcommand\comt{\mathsf{unit}}
\newcommand\expt{\mathsf{int}}
\newcommand\Z{\mathbb{Z}}
\newcommand\A{\mathbb{A}}
\newcommand\vart{\mathsf{XXX}}
\newcommand\val{\mathsf{Val}}
\newcommand\Sto{\mathsf{Sto}}
\newcommand\Av{\mathsf{Av}}
\newcommand\Sig{\Sigma}
\newcommand\rarr{\rightarrow}
\newcommand\boldemph[1]{\emph{\textbf{#1}}}
\newcommand\rnode{}
\newcommand\justf{}
\newcommand\justfs{}
\newcommand\ssl{}
\newcommand\seq{}
\newcommand\restg{}
\newcommand\nccdu{}
\newcommand\inter[1]{\mathsf{Inter}(#1)}
\newcommand\letin[2]{\mathsf{let}\ #1\ \mathsf{in} \ #2}
\newcommand\id{\mathsf{id}}
\newcommand\GOQ{\mathsf{OQ}}
\newcommand\GOA{\mathsf{OA}}
\newcommand\GPQ{\mathsf{PQ}}
\newcommand\GPA{\mathsf{PA}}
\newcommand\qd{}
\newcommand\GG{\mathcal{G}}

\section{LTS full abstraction}

\begin{definition}
An \emph{arena} $A=\ang{M_A,I_A,\lambda_A,\vdash_A}$ is given by:
\begin{itemize}
 \item a set of moves $M_A$ and a subset $I_A\subseteq M_A$ of initial ones,
 \item a labelling function $\lambda_A:M_A\to\{O,P\}\times\{Q,A\}$,
 \item a justification relation $\vdash_A\; \subseteq M_A\times(M_A\setminus I_A)$;
\end{itemize}
satisfying, for each $m,m'\in M_A$, the conditions:
\begin{itemize}
 \item $m\in I_A\implies \lambda_A(m)=(P,A)$,
 \item $m\vdash_A m'\land \lambda_A^{QA}(m)=A \implies \lambda_A^{QA}(m')=Q$,
 \item $m\vdash_A m' \implies \lambda_A^{OP}(m)\not=\lambda_A^{OP}(m')$.
\end{itemize}
\end{definition}

\medskip

The labelling function classifies moves as belonging to Opponent ($O$) or Proponent ($P$), and as questions ($Q$) or answers ($A$).
We range over moves by $m,n$ and use $\ini, \que, \ans$ to refer
to initial, question and answer moves respectively.
We also use $o$ and $p$ to stress ownership of moves.
Let $\overline{\lambda}_A$ be the OP-complement of $\lambda_A$.
Note that if $\ini\vdash_A m$ then $\lambda_A(m)=(O,Q)$.
%We call such moves $m$ the \emph{initial questions} of the arena $A$.

Given arenas $A,B$, the arenas  $A\otimes B$ and $A\To B$ 
are constructed as follows, where 
$\bar{I}_A=M_A\setminus I_A$, $\bar{\vdash}_A=(\,\vdash_A\rest \bar{I}_A{}^2)$
(and similarly for $B$).
\begin{align*}
 M_{A\otimes B} &= (I_A\times I_B)\uplus \bar{I}_A\uplus \bar{I}_B  \quad I_{A\otimes B} = I_A\times I_B \\
 \lambda_{A\otimes B} &= [(\ini_A,\ini_B)\mapsto PA,\, \lambda_A\rest\bar{I}_A,\, \lambda_B\rest\bar{I}_B]  \\
 \vdash_{A\otimes B} &= \{((\ini_A,\ini_B),m)\ |\ \ini_A\vdash_A m\lor \ini_B\vdash_B m\}\cup\bar{\vdash}_A\cup\bar{\vdash}_B
\\[2mm]
%\end{align*}
%\begin{align*}
 M_{A\To B} &= \{\star\}\uplus M_A\uplus M_B  \quad I_{A\To B} = \{\star\} \\
 \lambda_{A\To B} &= [\,\star\mapsto PA,\, \overline{\lambda}_A[\ini_A\mapsto OQ],\, \lambda_B]  \\
 \vdash_{A\To B} &= \{(\star,\ini_A)\}\cup\{(\ini_A,\ini_B)\}\cup \vdash_A \cup \vdash_B
\end{align*}
Now for each type $\theta$ we define the corresponding arena $\sem{\theta}$.
%
\begin{align*}
\sem{\comt} &= \ang{\{\star\},\{\star\},\emptyset,\emptyset} &
\sem{\expt} &= \ang{\Z,\Z,\emptyset,\emptyset} \\
\sem{{\theta}\times\theta'} &= \sem{\theta}\otimes\sem{\theta'} & 
\sem{\theta\to\theta'} &= \sem{\theta}\Rightarrow\sem{\theta'}
\end{align*}
We write $1$ for $\sem{\comt}$ and $\Z$ for $\sem{\expt}$.

Although types are interpreted by arenas, the actual games will be played in \emph{prearenas}, which
are defined in the same way as arenas with the exception that initial moves are O-questions. Given arenas $A,B$ we define the prearena $A\to B$ as follows.
\begin{align*}
 M_{A\to B} &= M_A\uplus M_B  & \lambda_{A\to B} &= [\overline{\lambda}_A[\ini_A\mapsto OQ],\lambda_B]  \\
 I_{A\to B} &= I_A &  \vdash_{A\to B} &= \{(\ini_A,\ini_B)\}\cup\vdash_A\cup\vdash_B
\end{align*}

\begin{definition}\normalfont
A \emph{justified sequence} on a prearena $A$ is a sequence of moves from $M_A$ such that, apart from the first move which must be from $I_A$, every move in $s$ is equipped with a pointer to an earlier move, called a \emph{justification pointers}, such that:
\begin{itemize}
 \item if $n$ points to $m$ 
 then either $m,n\in M_A$ and $m\vdash_A n$, 
 or $m,n\in M_{\theta\rarr\theta'}$ for some $\theta,\theta'$ 
 and $m\vdash_{\sem{\theta\rarr\theta'}} n$. 
 We say that $m$ \emph{justifies} $n$.
\end{itemize}
A justified sequence $s$ is called a \boldemph{play} if, in addition:
\begin{itemize}
\item no adjacent moves belong to the same player (\emph{Alternation});
\item the justifier of each answer is the most recent unanswered question (\emph{Bracketing});
\item for each prefix $s'm$ of $s$, with $s'\not=\varepsilon$, the justifier of $m$ is in $\view{s'}$ (\emph{Visibility)}.
\end{itemize}
 The \boldemph{view} of an  alternating justified sequence is given by:
  \[
    \begin{aligned}
      \view{s} &= s \text{\,, if $|s|\leq1$}\\
    \view{s'ns''m} &= \view{s'}nm \text{\,, if $n$ justifies $m$}
    \end{aligned}
  \]
  We write $P_A$ for the set of all plays on $A$
\end{definition}

Note that, because of visibility, when taking the view of a play we obtain a play, as all moves have their pointers retained.
From the notion of view we derive those of P-view ($\pview{s}$) and O-view ($\oview{s}$), defined as follows:
\begin{align*}
  \pview{s} &= \begin{cases} \view{s} & \text{ if $|s|$ is odd or $s=\varepsilon$}\\
    \view{s'}m & \text{ if $|s|$ is even and $s=s'm$}
  \end{cases}\\
    \oview{s} &= \begin{cases} \view{s} & \text{ if $|s|$ is even}\\
    \view{s'}m & \text{ if $|s|$ is odd and $s=s'm$}
    \end{cases}
  \end{align*}
So, in a play, when Proponent is next to make a move, the view of the current play is a P-view (as the current play is odd-length), and dually for Opponent. 

\begin{definition}\normalfont
A \boldemph{strategy} $\sigma$ on a prearena $A$, written $\sigma:A$, is a set of even-length plays of $A$ satisfying:
\begin{itemize}
\item if $sop\in\sigma$ then $s\in\sigma$ (\emph{Even-prefix closure});
\item if $sp_1,sp_2\in\sigma$ then $p_1=p_2$ (\emph{Determinacy});
\item if $s_1p,s_2\in\sigma$ and $s_2o$ a play such that $\view{s_1}=\view{s_2o}$ then $s_2op\in\sigma$ (\emph{Innocence}).
\end{itemize}
\end{definition}

\begin{remark}
  Intuitively, innocence ensures that the moves played by Proponent depend solely on his view of the play so far (the \emph{P-view}). In particular, if Proponent plays a particular move $p$ when the current play is $s_1$, then he must play $p$ in \emph{every} play that has the same view as $s_1$.

Note also that combining innocence with determinacy we obtain the following:
\begin{itemize}
\item if $s_1p_1,s_1p_2\in\sigma$ and $\view{s_1}=\view{s_2}$ then $p_1=p_2$.
\end{itemize}
The above can be seen as saying that Proponent's moves are \emph{determined} by his view of the play.
\end{remark}


We now turn to defining a suitable notion of interaction between plays.
Given arenas $A, B, C$, we define the prearena $A\to B\to C$ by setting $M_{A\to B\to C} = M_{A\to B}\uplus M_C$, $I_{A\to B\to C} = I_A$ and:
\[\begin{aligned}
\lambda_{A\to B\to C} &= [\lambda_{A\to B}[\ini_B\mapsto PQ],\overline{\lambda}_C] \\
\vdash_{A\to B\to C} &= {\vdash_{A\to B}} \cup\{(\ini_B,\ini_C)\} \cup \vdash_C 
\end{aligned}\]
Let $u$ be a justified sequence on $A\to B\to C$.
We define $u\upharpoonright AB$ to be $u$ in which all $C$-moves are suppressed.
$u\upharpoonright BC$ is defined analogously.
$u\upharpoonright AC$ is defined similarly with the caveat that, if there was a
pointer from
a $C$-move to a $B$-move which in turn had a pointer to an $A$-move, we add a
pointer from the $C$-move to the $A$-move.
Similarly, given a justified sequence $s$ on $A\to B$, we define the projections $s\rest A $ and $s\rest B$. 

\begin{definition}\normalfont
  Let $s\in P_{A\to B},t\in P_{B\to C}$ be such that $s\rest B=t\rest B$. We define their \emph{parallel composition} $s\|t$ by recursion as follows. We set $\varepsilon\|\varepsilon=\varepsilon$, and:
  \[
sm_A \| t = (s\|t)m_A \qquad
sm_B\|tm_B = (s \|t)m_B\qquad
s \| tm_C= (s\|t)m_C
 \] 
The composite of s and t is:
$
  s ; t = (s \| t)\rest AC .
  $\\
  The set of interaction sequences of $A, B, C$ is defined as:
  \[
    \inter{A,B,C}= \{s ; t | s \in P_{A\to B}, t \in P_{B\to C} , s\rest B=t\rest B\} .
\]
  \end{definition}

\begin{corollary}
For all $u\in\inter{A,B,C}$ we have $u\rest AB\in P_{A\to B}$ and $u\rest BC\in P_{B\to C}$. 
\end{corollary}

\begin{definition}
Given strategies $\sigma:A\to B$ and $\tau:B\to C$ we define 
the composite strategy $\sigma;\tau:A\to C$ to be
\begin{align*}
 \sigma;\tau  &= \{\,s;t\ |\ s\in\sigma,t\in\tau,s\rest B=t\rest B\,\}.
\end{align*}
\end{definition}

\begin{proposition}\label{p:welldef}
Strategy composition is well-defined, i.e.~for all $\sigma:A\to B$ and $\tau:B\to C$, $\sigma;\tau$ is a strategy on $A\to C$.
\end{proposition}

\begin{proposition}\label{p:assoc}
Composition of strategies is associative.
\end{proposition}

\begin{definition}
$\GG$ is the category of arenas and strategies, in which
strategies in the prearena $A\to B$ are morphisms between $A$ and $B$.
\end{definition}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> typing.tex <==
\section{Typing rules of \lang}\label{sec:typing}

\newcommand\qweqwe{\quad}
\newcommand\preG[1][]{\Delta#1;\varSigma\vdash}
\newcommand\atype[1]{\mathsf{#1}}
\newcommand\vars{Vars}
\newcommand\refs{Refs}
\newcommand\meths{Meths}

\begin{gather*}
%=====Unit=====
{\infer{c\text{ cons.\ of type }T}{ \preG c : T }}
\qweqwe
%=====Variables=====
\infer{ (x:T)\in\Delta }{ \preG x : T }
\qweqwe
%=====Tuples=====
\infer{ \preG e_1: T_1\quad\dots\quad \preG e_n: T_n }{ \preG (e_1,\dots,e_n) : T_1*\dots*T_n }
\\[1mm]
%=====Ops=====
\infer{ op:\vec T\to T\quad  \preG (\vec e):\vec T }{ \preG \arithop{\vec e} : T }
\qweqwe
%=====Conditionals=====
\infer{ \preG e : \atype{bool}\qquad  \preG (e_1,e_2) : T*T }{ \preG \cond{e}{e_1}{e_2} : T }
\\[1mm]
%=====New=====
\infer{\preG v : T \quad  \Delta;\varSigma,l:T\vdash e : T' }{ \preG \new l v e : T' }
\qweqwe 
%=====Dereferencing=====
\infer{ (l:T)\in\varSigma }{ \preG {!l} : T }
\qweqwe
% =====Assigning=====
\infer{ (l:T)\in\varSigma \quad \preG e : T }{\preG l := e : \atype{unit} }
\\[1mm]
%=====Function Application=====
\infer
{ \preG e: T \rightarrow T' \quad \preG e' : T }
{ \preG ee' : T' }
\qweqwe 
%=====fix bindings=====
\infer{ \preG[,f:T\to T',x:T] e : T' }{ \preG \lam{x}{e} : T\to T'}
\\[1mm]
%=====Let bindings=====
\infer{ \preG[,x_1:T_1,\dots,x_n:T_n] e : T \quad  \preG e' : \vec T }{ \preG \elet{(\vec x)}{e'}{e} : T }
\end{gather*}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

